Unsupervised Information Obfuscation for Split Inference of Neural Networks

Splitting network computations between the edge device and a server enables low edge-compute inference of neural networks but might expose sensitive information about the test query to the server. To address this problem, existing techniques train the model to minimize information leakage for a given set of sensitive attributes. In practice, however, the test queries might contain attributes that are not foreseen during training. We propose instead an unsupervised obfuscation method to discard the information irrelevant to the main task. We formulate the problem via an information theoretical framework and derive an analytical solution for a given distortion to the model output. In our method, the edge device runs the model up to a split layer determined based on its computational capacity. It then obfuscates the obtained feature vector based on the first layer of the server model by removing the components in the null space as well as the low-energy components of the remaining signal. Our experimental results show that our method outperforms existing techniques in removing the information of the irrelevant attributes and maintaining the accuracy on the target label. We also show that our method reduces the communication cost and incurs only a small computational overhead.

==> 5_experiments_old.tex <==
% \vspace{-0.25cm}
\section{Experimental Results}\label{sec:experiment}
% \vspace{-0.25cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Experiment Setup}

\noindent{\bf Model architecture and training settings.} We present the experimental results on an architecture used in prior work~\citep{song2019overlearning} which is shown in Table~\ref{tab:architecture}. We use the same architecture for adversary's model $M_a$ as the server model $M_s$. 
We train the models for $50$ epochs using the Adam optimizer with an initial learning rate of $0.001$. The learning rate is dropped by a factor of $10$ after $20$ and $40$ epochs. 



\noindent{\bf Datasets.} We perform our experiments on four visual datasets described below. Table~\ref{tab:baseline-accs} lists the target and hidden attributes of the datasets used. 
\begin{itemize}[itemsep=2pt,leftmargin=0.5cm]
    \item {\bf EMNIST}~\citep{cohen2017emnist} is an extended version of the MNIST dataset where the labels are augmented with writer IDs. 
    % To have a uniform distribution of writer identities, 
    We select $13000$ samples from EMNIST written by $100$ writers with $130$ examples per writer. We then split this dataset into $10000$, $1500$, and $1500$ for training, validation, and testing. We use the digit label and the writer ID as the target and the hidden attributes, respectively. 
    
    \item {\bf FaceScrub}~\citep{facescrub2,facescrub} is a dataset of celebrity faces labeled with gender and identity. We use gender as the target and identity as the hidden attribute. In experiments, we crop images using the face region bounding boxes specified in the annotations and resize them to $50\times 50$.
    
    \item {\bf UTKFace}~\citep{utkface} is a dataset of face images labeled with gender and race, which we treat as the target and the hidden attributes, respectively. The images are cropped using the face region bounding boxes and resized to $50\times 50$.
    
    \item {\bf CelebA}~\citep{celeba} is a dataset of celebrity images. Each image is labeled with 40 binary attributes, out of which, we select \emph{Smiling} as the target attribute and \{\emph{Male}, \emph{Heavy\_Makeup}, \emph{High\_Cheekbones}, \emph{Mouth\_Slightly\_Open}, \emph{Wearing\_Lipstick, Attractive}\} as hidden attributes. These attributes have near balanced distribution of positive and negative examples. 
    In experiments, we crop images to the face region and resize them to $73\times 60$.
\end{itemize}


\begin{table}[t]
\centering\small
\caption{\small Network Architecture. Each row shows a  split layer, i.e., 
for the split layer $i$, the input of that layer is sent to the server.}\label{tab:architecture}
\vspace{-0.1cm}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{cl}
\toprule
{\textbf{Layer}}  & \textbf{Architecture} \\ 
\midrule
{\small \textbf{1}}  & {\small CONV($3,16$), ReLU, Maxpool($2\times 2$), Batchnorm} \\
{\small \textbf{2}}  & {\small CONV($3,32$), ReLU, Maxpool($2\times 2$), Batchnorm} \\
{\small \textbf{3}}  & {\small CONV($3,64$), ReLU, Maxpool($2\times 2$), Batchnorm} \\
{\small \textbf{4}}  & {\small FC(128), ReLU, Batchnorm} \\
{\small \textbf{5}}  & {\small FC(64), ReLU, Batchnorm} \\
{\small \textbf{6}}  & {\small FC($n_{\mbox{\tiny classes}}$), Softmax} \\
\bottomrule
\end{tabular}
%}
% \vspace{-0.25cm}
\end{table}


% \begin{table*}[h]
% \caption{\small Model accuracy for target and hidden attributes of different datasets.}\label{tab:baseline-accs} 
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l c c c cccccc}
% \toprule
% \textbf{Dataset}               & MNIST  & UTKFace & FaceScrub & \multicolumn{6}{c}{CelebA}                                        \\ 
% \midrule
% \textbf{Target attribute}      & digit  & gender  & gender    & \multicolumn{6}{c}{smiling}                                       \\
% \textbf{Number of classes}           & 10     & 2       & 2         & \multicolumn{6}{c}{2}                                             \\
% \textbf{Target accuracy (\%)}  & 98.60  & 90.25   & 97.90     & \multicolumn{6}{c}{92.25}                                         \\
% \midrule
% \textbf{Hidden attribute}     & writer & race    & identity  & gender & makeup & cheekbones & mouth-open & lipstick & attractive \\
% \textbf{Number of classes}           & 100    & 5       & 530       & 2      & 2      & 2          & 2          & 2        & 2          \\
% \textbf{Attack accuracy (\%)} & 26.93  & 79.18   & 65.52     & 97.53  & 90.00  & 86.29      & 92.94      & 93.40    & 80.46 \\
% \bottomrule
% \end{tabular}
% }
% %\vspace{-0.25cm}
% \end{table*}

\begin{table*}[t]
\caption{\small Target and hidden attributes of the datasets used.}\label{tab:baseline-accs} 
\vspace{-0.1cm}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c cccccc}
\toprule
\textbf{Dataset}               & MNIST  & UTKFace & FaceScrub & \multicolumn{6}{c}{CelebA}                             \\ 
\midrule
\textbf{Target attribute}      & digit  & gender  & gender    & \multicolumn{6}{c}{smiling}                            \\
\textbf{Number of classes}           & 10     & 2       & 2         & \multicolumn{6}{c}{2}                            \\
\midrule
\textbf{Hidden attribute}     & writer & race    & identity  & gender & makeup & cheekbones & mouth-open & lipstick & attractive \\
\textbf{Number of classes}           & 100    & 5       & 530       & 2      & 2      & 2          & 2          & 2        & 2          \\
\bottomrule
\end{tabular}
}
%\vspace{-0.25cm}
\end{table*}


\noindent{\bf Measuring obfuscation.} 
Several methods have been proposed to measure the information leakage of intermediate feature vectors in neural networks. One approach is computing the mutual information between the query $x$ and the feature vector $z'$~\citep{kraskov2004estimating}. In practice, measuring the mutual information is not tractable for high-dimensional random variables, unless certain assumptions are made about the probability distribution of the random variables of interest. A more practical approach computes the reconstruction error, $\|\widetilde{x}-x\|$, where $\widetilde{x}$ is estimated using the feature vector~\citep{mahendran2015understanding}. Finally, attribute leakage can be defined based on the accuracy of an adversary model that predicts the hidden label from intermediate features. 

% In our threat model, the server only knows $y^\pub$ and can only use this information to train $M_s\circ M_c$. 
% At the inference phase, the client computes $z=M_c(x)$ locally and queries the server, which computes $y^{pub}=M_s(z)$.


% In this paper, our goal is to minimize the leakage of hidden attributes without the knowledge of those attributes. 
In this paper, we follow the approach of predicting hidden attributes using an adversary model. 
Assume that each example $\{x_i\}_{i=1}^N$ has a target label $\{y^\pub_i\}_{i=1}^{N}$ and a hidden label $\{y^{\pri}_i\}_{i=1}^N$. 
The adversary trains the model $M_a$ with $(z'_i, y_i^\pri)$, where $z'_i=g(M_c(x_i))$ is the same feature vector that the server also receives to do inference of the target label.
Note that the training of $M_a$ is used as a post hoc process to evaluate the leakage of sensitive attributes and does not influence the client or server's processing. 
We refer to the accuracy of $M_s \circ g \circ M_c$ on $y^{\pub}$ as \emph{target accuracy} and the accuracy of $M_a \circ g \circ M_c$ on $y^{\pri}$ as \emph{attack accuracy}. 




% \noindent{\bf Client, server, and adversary assumptions. } We assume that the server trains $M_s\circ M_c$ using only training data and public labels.
% Note that the server is willing to cooperate in providing a privacy-preserving model that only extracts intended attributes. This is a viable scenario as providing privacy gives competitive advantage to different companies providing a similar service. 
% After training, the server and client may agree to split the inference at different layers. The adversary utilizes the output of $M_c$ to infer private labels. 

% \noindent{\bf Adversary capabilities.} We use the same architecture for adversary's model $M_a$ as the server model $M_s$. 
% The model $M_a$ is trained using the features extracted by $M_c$ and the associated private labels. We also assume that the adversary knows the parameters of $M_c$ and $M_s$. %, which makes him capable of extracting signal space content from noisy features. 
% The adversary cannot change the parameters of $M_c$ or $M_s$.





\subsection{Evaluations}\label{sec:content}



% \hh{in some cases (particularly EMNIST in Figure 5), public accuracy seems to take a larger hit than the private one. This can happen and we cannot control over}

% \hh{we do comparisons with AT because it provides the best tradeoff of accuracy and obfuscation compared to others, including adding noise and IB}

% \hh{More explanation is need about adversarial training in the evaluation section. 
% My understanding from the current text is that it is only trained to obfuscate one attribute (gender), but what if we train it to obfuscate more attributes? }

% \noindent{\bf Baselines.} The baseline test accuracy results are provided in Table~\ref{tab:baseline-accs}. Note that the accuracy on hidden attributes could be higher or lower than the target accuracy depending on the difficulty of the tasks. We do not compare these two quantities. Instead, we compare different methods in how much they reduce the attack accuracy, while maintaining the target accuracy.


\noindent{\bf Cumulative signal content.} 
We start our analysis by computing the norm of the null and signal contents in every layer of $M = M_s \circ M_c$. At each layer, the null content $z_\mathcal{N}$ is discarded and the signal content $z_\mathcal{S}$ is passed through the next layer. We compute the normalized amount of the information passed from the $i$-th layer to the next as $C_{\mathcal{S}}(z^{(i)})=\log(\frac{\|z_{\mathcal{S}}^{(i)}\|_2^2}{\|z^{(i)}\|_2^2})$, where $z^{(i)}$ and $z_{\mathcal{S}}^{(i)}$ are the activation vector and its signal content at the $i$-th layer, respectively.
% The normalized signal and null contents of $z$ are defined as $C_{\mathcal{S}}(z)=\frac{||z_{\mathcal{S}}||_2^2}{||z||_2^2}$ and $C_{\mathcal{N}}(z)=\frac{||z_{\mathcal{N}}||_2^2}{||z||_2^2}$, respectively.
% Recall that the signal-space and null-space content ($C_{\mathcal{S}}(z)$ and $C_{\mathcal{N}}(z)$) are in range $[0,1)$ defined in Section~\ref{sec:training}.
% \edit{For CONV layers, we compute $C_{\mathcal{N}}(z)$ for every $z$ that is obtained from a sliding window, then report the average of $C_{\mathcal{N}}(z)$ for all windows.} 
Figure~\ref{fig:baseline} shows the cumulative amount of the signal content preserved up to the $i$-th layer, computed as $\sum_{j=1}^{i}C_{\mathcal{S}}(z^{(j)})$. 
% As can be seen, the main network inherently discards information irrelevant to $y^\pub$ from one layer to the next, until the prediction is made at the last layer. 
The plot suggests that the model gradually removes the content irrelevant to the target label from one layer to the next, thus acting as an obfuscator. 

% and $C_{\mathcal{S}}(\cdot)$ is presented in Definition~\ref{def:normalized_content}.
% signal and null contents for all layers across the evaluated datasets. As seen, features contain null-space content that is filtered out when the next layer is applied. 
% As the feature vector propagates through network layers, more content is gradually removed from $z$ until the model outputs the prediction on the main task. 



\begin{figure}[h]
    \centering
    % \vspace{-0.1cm}
    \includegraphics[width=0.4\linewidth]{Figures/signal_content_HH.png}
    % \vspace{-0.1cm}
    \caption{\small Cumulative preserved signal content at different layers of the model $M_s\circ M_c$. 
    The model acts as an obfuscator, gradually removing the content irrelevant to the target label from one layer to the next.}
    \label{fig:baseline}
    % \vspace{-0.25cm}
\end{figure}

\begin{figure*}[t]
    \centering
    % \vspace{-0.1cm}
    \includegraphics[width=\textwidth]{Figures/tradeoff7.png}
    % \vspace{-0.3cm}
    \caption{\small Attack accuracy versus the split layer for three settings: (1)~baseline network without data obfuscation, (2)~distortion-free obfuscation, and (3)~distortion-bounded obfuscation with at most $1\%$ drop in target accuracy.
    % The effect of the split layer and our proposed methods for filtering features vector on private accuracy. The Y-axis in each figure covers the range between random guess and the baseline accuracy. 
    % Removing the null content reduces the private accuracy without affecting the public accuracy. Also, removing part of the signal content further reduces the private accuracy, in some cases to the level of random guess, while slightly reducing the public accuracy.
    % The total number of features is $m=16$. 
    % For a given split layer, the number of preserved features ($m'$) can be tuned so as to achieve a desired tradeoff between utility (higher public accuracy) and privacy (lower private accuracy). Also, better tradeoffs can be achieved when the network is split from deeper layers.
    }\label{fig:private_acc_layers}
    % \vspace{-0.25cm}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.4\columnwidth]{Figures/Example-Tradeoff.png}
    \caption{\textcolor{red}{\small Tradeoff between utility and obfuscation for the UTKFace dataset, when the network is split at the input of the FC1 layer. As we increase the number of preserved features ($m'$), utility is increased (lower target error) but obfuscation is decreased (lower attack error).}}
    \label{fig:ex_m_prime}
\end{figure}


\begin{figure*}[t]
% \vspace{-0.1cm}
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/comparison_pruning.png}
    % \vspace{-0.4cm}
    \caption{\small Comparison between our method and feature pruning. The horizontal and vertical axes show the classification \textbf{error} on $y^\pub$ and $y^\pri$, respectively. Our goal is to have low error on $y^\pub$ and high error on $y^\pri$. In most cases, our method significantly outperforms feature pruning, i.e., with the same utility (target error), our method achieves better obfuscation (higher attack error). For CelebA, the sensitive attribute in this study is ``gender''.}
    \label{fig:pub-priv-tradeoff}
    % \vspace{-0.5cm}
\end{figure*}


\noindent{\bf Investigating tradeoffs.} 
% We now evaluate the information leakage based on the attack accuracy. 
% The information leakage is considered high if the adversary can train a model $M_a$ that accurately estimates $y^\pri$. 
% In the remainder, we use the adversary (attack) accuracy as a proxy to information leakage.
% As such, it is safe to assume that the features become more related to the public task as we move towards the last layer. We next test this hypothesis by cutting the network at different layers and extracting private attributes from the features.
Figure~\ref{fig:private_acc_layers} shows the attack accuracy versus the split layer for three settings: (1)~without obfuscation, (2)~with distortion-free obfuscation (i.e., when $m'=m$), and (3)~with distortion-bounded obfuscation such that the drop in target accuracy is at most $1\%$. The results illustrate the tradeoffs between edge computation, obfuscation, and target accuracy, described in the following.
\begin{itemize}[itemsep=2pt,leftmargin=0.5cm]%[leftmargin=*]
    \item In all three cases, the attack accuracy decreases as the network is split at deeper layers. This observation indicates that more edge computation results in lower attack accuracy at the same target accuracy. 
    \item For each split layer, the attack accuracy of distortion-free obfuscation is less than that of baseline. This observation shows that even without decreasing the target accuracy, the feature vector can be modified to obtain a better obfuscation. 
    
    \item For each split layer, the distortion-bounded obfuscation further reduces the attack accuracy at a small reduction of at most $1\%$ in target accuracy. \textcolor{red}{For the same split layer (same edge compute), the number of preserved features, $m'$, provides a tradeoff between the target accuracy and obfuscation. We show an example of this effect in Figure~\ref{fig:ex_m_prime}.}
\end{itemize}




% for different split layers. As can be seen, the attack accuracy decreases as the model is split in layers closer to the output. 
% The observations provided by Figure~\ref{fig:baseline} indicate that the content discarded by the model from one layer to the next contained information relevant to the hidden attribute and, thus, the model itself acts as an obfuscator. 
% , gradually removing the content irrelevant to the target label .
% This observation indicates that the content discarded by the previous layers contained information relevant to the hidden attribute.

% \noindent{\bf Attacking baseline network.} We split the main network (trained on the public task) at different layers, construct the adversary network as $M_a\circ M_c$, and train the adversary network using private labels.
% % \edit{For this task, the weights of $M_c$ are fixed and only $M_a$ is trained.} 
% The accuracy of $M_a$ for each dataset at each layer is shown in Figure~\ref{fig:baseline}~(right). If we split the network in deeper layers, the accuracy of $M_a$ drops. This verifies our hypothesis that information about the private attribute is thrown away from one layer to the next. However, even at the last layer, the private accuracy is still relatively high, meaning that the the network is not necessarily filtering out \textit{all} the private information.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{Figures/baseline_private.png}
%     \vspace{-0.3cm}
%     \caption{ The adversary is trained on the features that are input to each split layer.}
%     \label{fig:private-baseline}
%     \vspace{-0.3cm}
% \end{figure}


% \begin{wrapfigure}[16]{R}{0.4\columnwidth}
% \vspace{-0.5cm}
% \begin{figure}
% \centering
% \includegraphics[width=0.75\columnwidth]{Figures/same_pub.png}
% % \vspace{-0.15cm}
%     \caption{\small 
%     % Private accuracy when satisfying public accuracy of 97\% for EMNIST, 90\% for UTKFace, 97\% for FaceScrub, and 90\% for CelebA.
%     Attack accuracy versus split layer. The number of preserved components of signal content is set such that the target accuracy is reduced by $1\%$. \mohammad{merge with Fig-3}}
%     \label{fig:same_pub}
% \end{figure}
% \vspace{-.1cm}
% \end{wrapfigure}




% \noindent{\bf Privacy-preserving inference.} 
% Next, we demonstrate the effect of distortion-free obfuscation on the information leakage. It works by filtering out the null content of the feature vector. Figure~\ref{fig:top-bot} shows the attack accuracy for different split layers. Removing the null content reduces the attack accuracy without affecting the target accuracy. Moreover, splitting the network in deeper layers appears to reduce the information leakage indicated by the drop in adversary's accuracy.


% To further reduce the information leakage, we discard the low-energy components of the signal content and only keep $m'$ features.




% Better tradeoffs can be achieved when the network is split from deeper layers, i.e., the edge device performs more computation. \edit{Note that the notion of feature is different for CONV and FC layers, that is, the $m'$ required to preserve the public accuracy is not necessarily the same in all layers. We show the private accuracy when a certain public accuracy is to be satisfied in Figure~\ref{fig:same_pub}.}
% Figure~\ref{fig:top-bot} shows that the information leakage can be controlled using the following factors: 
% \begin{itemize}[itemsep=4pt,leftmargin=0.75cm]%[leftmargin=*]
    % \item {\bf Number of signal components sent to the server:} For the same edge-computation (a given split layer), the number of preserved features ($m'$) can be tuned so as to achieve a desired tradeoff between utility (higher public accuracy) and privacy (lower private accuracy). 
    
    % \item {\bf The split layer:} Better tradeoffs can be achieved when the network is split from deeper layers, i.e., the edge device performs more computation. \edit{Note that the notion of feature is different for CONV and FC layers, that is, the $m'$ required to preserve the public accuracy is not necessarily the same in all layers. We show the private accuracy when a certain public accuracy is to be satisfied in Figure~\ref{fig:same_pub}.}
% \end{itemize}


% Removing the null-space content ($z_{\mathcal{N}}$) reduces the private accuracy without sacrificing the public accuracy.  One can reduce the private information leakage by further removing content from the signal space, which come at the cost of reduced public accuracy. 
% Comparing the top and bottom rows of Figure~\ref{fig:top-bot}, 
% The drop in public accuracy can be negligible if enough features ($m'$) are kept in the signal content. At the same time, the private accuracy drops significantly and gets close to random guess. 








% We illustrate the utility-privacy tradeoff in Figure~\ref{fig:pub-priv-tradeoff} (top); Here, we split the network halfway in the middle, i.e., at the input of $FC$-1.  As seen, our method allows to have a high public accuracy with relatively small $m'$, which results in a low private accuracy.




\noindent{\bf Comparison to pruning.} Similar to our approach, pruning network weights eliminates features that do not contribute to the classification done by $M_s$. \textcolor{red}{Since pruning does not require access to the sensitive labels, it is a natural unsupervised obfuscation baseline.}
In the following, we compare our method with pruning in terms of target and attack accuracy. We split the network at the middle layer, i.e., the input of the $FC1$ layer. For our method, we keep the top $m'$ components of $z$ from its signal content and filter out the rest. For pruning, we keep $m'$ elements in $z$ and set the rest to zero. We adopt the pruning algorithm proposed by~\citep{li2016pruning} which works based on the $L_1$ norm of the columns of the following layer's weight matrix. After pruning, we fine-tune $M_s$ to improve its accuracy. \textcolor{red}{By changing $m'$, we achieve a tradeoff between attack and target error for pruning and our own method, and show the resulting tradeogg in Figure~\ref{fig:pub-priv-tradeoff}. In this figure, points with higher attack error and lower target errors are desired. As seen, our method achieves a better tradeoff compared to pruning. This is an after effect of minimizing the distortion to the target accuracy while maximizing the obfuscated ``unrelated'' information in our method.}
% \textcolor{red}{ shows the accuracy of the main model and the adversary for each dataset. 
% As seen, with small $m'$, both our method and pruning achieve low attack accuracy. Pruning, however, significantly reduces the target accuracy as well. For example, for the UTKFace dataset, with $m'=1$, both methods result in the attack accuracy close to a random guess. However, pruning reduces the target accuracy from $92.25\%$ to $53\%$ (similarly close to random guess), whereas our method yields $88.63\%$ accuracy.

% we apply pruning on the inputs of the split layer and show the utility-privacy tradeoff in Figure~\ref{fig:pub-priv-tradeoff} (bottom). We take the weight matrix of the first layer of $M_s$, and prune the transmitted features according to the sum of absolute values in the columns of the matrix~(\citep{li2016pruning}). 
% As seen in Figure~\ref{fig:pub-priv-tradeoff} (bottom), pruning successfully reduces the private accuracy; however, the privacy achieved by pruning comes at the cost of a significant degradation in utility. Take the UTKFace task as an example; with $m'=1$ features, both our method and pruning result in a private accuracy  close to the random guess ($42.84\%$). However, pruning reduces the public accuracy from $92.25\%$ to $53\%$ (also close to random guess for the public task), whereas our method keeps the public accuracy at $88.63\%$.



\noindent{\bf Comparison with adversarial training.} \textcolor{red}{Among prior work in supervised data obfuscation, adversarial training is the natural baseline.} We compare our method to adversarial training, which generally provides the best tradeoff of accuracy and obfuscation compared to other methods such as information bottleneck~\citep{osia2018deep, moyer2018invariant} and noise injection~\citep{mireshghallah2020shredder}. 
We implemented the adversarial training framework proposed by~\citep{feutry2018learning} and trained the models in multiple settings with different $\gamma$ parameters (Eq.~\ref{eq:adversarial}) in range of $[0.1, 1]$ to achieve the best performance. 
Figure~\ref{fig:adversarial} shows the tradeoff between utility and obfuscation by measuring how much the attack error increases when target error is increased by a given value. 
% \edit{The network architecture for $M_c, M_s, M_a$ for the adversary is the same as those evaluated by our own method.} 
Note that, unlike our method, adversarial training assumes the hidden attribute is known at training time. Despite this, Figure~\ref{fig:adversarial} shows that, in most cases, our method significantly outperforms adversarial training, i.e., our method achieves better obfuscation (higher attack error) with the same utility (target error). 

\begin{figure*}[t]
% \vspace{-0.1cm}
    \centering
    % \includegraphics[width=0.9\textwidth]{Figures/publicVsprivate2.png}
    \includegraphics[width=\textwidth]{Figures/publicVsprivate_error.png}
    % \vspace{-0.4cm}
    \caption{\small Comparison between our method and adversarial training. The horizontal and vertical axes show the classification \textbf{error} on $y^\pub$ and $y^\pri$, respectively. Our goal is to have low error on $y^\pub$ and high error on $y^\pri$. In most cases, our method significantly outperforms adversarial training, i.e., with the same utility (target error), our method achieves better obfuscation (higher attack error). For CelebA, the sensitive attribute in this study is ``gender''.}
    \label{fig:adversarial}
    % \vspace{-0.2cm}
\end{figure*}


\begin{figure}[t]
    % \vspace{-0.1cm}
    \centering
    \includegraphics[width=0.6\columnwidth]{Figures/adversarial_multiple_3.png}
    % \vspace{-0.2cm}
    \caption{\small Accuracy on the target (\emph{Smiling}) and hidden attributes. 
    Our method obfuscates the feature vector without the knowledge of hidden attributes at training or inference times. Adversarial training (AT) method 
    maximizes the accuracy on \emph{Smiling}, while minimizing the accuracy on \emph{Gender}.
    As seen, AT successfully reduces accuracy on \emph{Gender} attribute but, unlike our method, fails to obfuscate information of other attributes. This highlights the applicability of our method in practical settings as a generic obfuscator compared to specialized techniques such as AT. }
    \label{fig:multi-private}
    % \vspace{-0.5cm}
\end{figure}

% \noindent{\bf Multiple private attributes.} 
% To highlight the independence of our method from private attributes,
We also do the experiments with multiple (unseen) hidden labels. Specifically, we consider the CelebA model trained to detect \emph{Smiling} and evaluate two methods, (1) our method: we keep only $m'=1$ component from the signal content of feature vector and then train one separate adversary model per hidden attribute, and (2) adversarial training: we first adversarially train an $M_c$ model to obfuscate \emph{Gender}, and then train one separate adversary model to predict each hidden attribute.

For both of the above methods, the network is split at the input of the $FC1$ layer. As shown in Figure~\ref{fig:multi-private}, our method outperforms adversarial training in both the target and attack accuracy. Specifically, our method results in a significantly lower attack accuracy on all hidden attributes compared to the baseline attack accuracy. The only exceptions are \emph{High\_Cheekbones} and \emph{Mouth\_Open} attributes, which highly correlate with the target attribute (a smiling person is likely to have high cheekbones and open mouth). The correlation between target and hidden attributes causes the signal content of the server and adversary models to have large overlaps and, hence, results in high attack accuracy. 
Also, as seen, the adversarially trained model successfully hides the information that it has been trained to obfuscate (\emph{Gender}). The model, however, fails to remove information of other attributes such as \emph{Makeup} or \emph{Lipstick}. The results highlight the importance of the generic unsupervised obfuscation in scenarios where the sensitive attributes are not known. In such cases, unlike supervised obfuscation methods, our method successfully reduces the information leakage.






%  \noindent {\bf Removing Null Content.} To reduce the amount of private information leakage, we apply null-space filtering~(Section~\ref{sec:null_filter}), as well as filtering the signal space content~(Section~\ref{sec:signal_filter}). The results are shown in Figure~\ref{fig:defended}. As seen, there are two factors contributing to the private accuracy: (i)~The split layer, and (ii)~the number of features that are preserved in the signal space (rank). The split layer specifies a tradeoff between client computation and privacy. The number of preserved features (when removing content from signal-space) specifies a tradeoff between utility and privacy. We present the public accuracy for each dataset in Figure~\ref{fig:public_accs}. Note that the amount of reduction in public accuracy is far less than the reduction in the private one. To give a more concrete analysis, we provide the public and private accuracies in Table~\ref{tab:public_private}. For brevity, we only show the case with the split layer placed halfway through the network (FC-1) and $m'=4$ features preserved from the signal-space. 
 
 
 

 
%  \begin{figure}[h]
%      \centering
%      \includegraphics[width=\columnwidth]{Figures/private_accs.jpg}
%      \caption{Accuracy of the adversary when extracting private information at different layers. The blue curve (baseline) shows the accuracy for unprotected features. The orange curve (null-removed) corresponds to the case where $z_{\mathcal{N}}$ is cleansed from features. The yellow, violate, and green curves show the accuracy when the signal-space content is also removed ($m'$ is the number of preserved features).}
%      \label{fig:defended}
%  \end{figure}
 
 
%   \begin{figure}[h]
%      \centering
%      \includegraphics[width=\columnwidth]{Figures/public_accs.jpg}
%      \caption{Accuracy of the main model when removing signal-space content at different layers. The accuracies are obtained after fine-tuning $M_s$ (the server's model) while $M_c$ parameter are frozen).}
%      \label{fig:public_accs}
%  \end{figure}
 
 
%  \begin{table}[h]
%  \centering
%  \caption{Changes in public and private attribute accuracy when $m'=4$ features are preserved from signal-space at layer \textit{FC-1}. The ``Random'' column shows the accuracy of a classifier that always predicts the label with maximum samples.}\label{tab:public_private}
%  \resizebox{0.9\columnwidth}{!}{
% \begin{tabular}{c|ccc|ccc}
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{Public Accuracy (\%)}}                                                  & \multicolumn{3}{c}{\textbf{Private Accuracy (\%)}}                         \\
%                                   & \textbf{Attribute}       & \textbf{Random  (\%)}  & \textbf{Change}                            & \textbf{Attribute} & \textbf{Random (\%)} & \textbf{Change}           \\ \hline
% \textbf{EMNIST}                   & digit                    & 10                     & 98.6$\rightarrow$91.7                    & author             & 1                    & 19.23$\rightarrow$3.9   \\ \hline
% \textbf{UTKFace}                  & gender                   & 53.03                  & 90.25$\rightarrow$89.36                  & race               & 42.84                & 76.98$\rightarrow$48.57 \\ \hline
% \multirow{6}{*}{\textbf{CelebA}}  & \multirow{6}{*}{smiling} & \multirow{6}{*}{52.03} & \multirow{6}{*}{92.25$\rightarrow$92.26} & gender             & 58.08                & 95.81$\rightarrow$64.47 \\
%                                   &                          &                        &                                            & makeup             & 61.57                & 88.17$\rightarrow$67.14 \\
%                                   &                          &                        &                                            & cheekbones         & 54.76                & 86.05$\rightarrow$83.55 \\
%                                   &                          &                        &                                            & mouth-open         & 51.78                & 89.49$\rightarrow$80.04 \\
%                                   &                          &                        &                                            & lipstick           & 53.04                & 91.71$\rightarrow$63.55 \\
%                                   &                          &                        &                                            & attractive         & 51.36                & 79.16$\rightarrow$61.8 
% \end{tabular}
% }
% \end{table}




% \noindent{\bf Comparison to Prior Work.} \textcolor{red}{We compare our method against adversarial training, which assumes that the private labels are known and are used for censoring private attributes. Table~\ref{tab:comparison} compares our method with~\citep{}, for which the authors provide codes.}

%  \begin{table}[h]
%  \centering
%  \textcolor{red}{
%  \caption{Comparison to prior work when splitting the network in the middle layer (FC-1). }\label{tab:comparison}
%  \resizebox{0.9\columnwidth}{!}{
% \begin{tabular}{c|ccc|ccc}
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{Public Accuracy (\%)}}                                                  & \multicolumn{3}{c}{\textbf{Private Accuracy (\%)}}                         \\
%                                   & \textbf{Attribute}       & \textbf{Adv.  (\%)}  & \textbf{ours}                            & \textbf{Attribute} & \textbf{Adv. (\%)} & \textbf{Ours}           \\ \hline
% \textbf{EMNIST}                   & digit                    & 10                     & 98.6$\rightarrow$91.7                    & author             & 1                    & 19.23$\rightarrow$3.9   \\ \hline
% \textbf{UTKFace}                  & gender                   & 53.03                  & 90.25$\rightarrow$89.36                  & race               & 42.84                & 76.98$\rightarrow$48.57 \\ \hline
% \multirow{6}{*}{\textbf{CelebA}}  & \multirow{6}{*}{smiling} & \multirow{6}{*}{52.03} & \multirow{6}{*}{92.25$\rightarrow$92.26} & gender             & 58.08                & 95.81$\rightarrow$64.47 \\
%                                   &                          &                        &                                            & makeup             & 61.57                & 88.17$\rightarrow$67.14 \\
%                                   &                          &                        &                                            & cheekbones         & 54.76                & 86.05$\rightarrow$83.55 \\
%                                   &                          &                        &                                            & mouth-open         & 51.78                & 89.49$\rightarrow$80.04 \\
%                                   &                          &                        &                                            & lipstick           & 53.04                & 91.71$\rightarrow$63.55 \\
%                                   &                          &                        &                                            & attractive         & 51.36                & 79.16$\rightarrow$61.8 
% \end{tabular}
% }
% }
% \end{table}

% \noindent{\bf Learning null-free features}
% % In our previous analysis, we showed that the leakage in private information can be controlled by elliminating content from the signal space of features.
% In the remainder of our analysis, we would like to see whether we can train the neural network such that the features automatically fall in the signal space. If this happens, the client would not be required to perform extra work to manually filter-out the null-content. Given a pre-trained $M=M_s\circ M_c$, we freeze $M_s$, and fine-tune $M_c$ via the loss function given in Equation~(\ref{eq:loss}), with $\gamma=1$. The results are shown in Table~\ref{tab:loss}. As seen, $M_c$ can be trained to censor null content automatically, ultimately reducing the private accuracy. 
% \begin{table}[h]
% \caption{Public and Private accuracy when the network is fine-tuned via Eq.~(\ref{eq:loss}) to censor the null content. The split layer is \textit{FC-3} in this experiment. Values before and after the arrow show the accuracy of the baseline model and fine-tuned model, respectively.} \label{tab:loss}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|c|c|c|cccc}
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{EMNIST}  & \multirow{2}{*}{UTKFace}  & \multirow{2}{*}{FaceScrub} & \multicolumn{4}{c}{CelebA}                                                                                    \\
%                          &                          &                           &                            & gender                    & makeup                    & lipstic                   & attractive                \\ \hline
% Public Accuracy          & 98.6$\rightarrow$98.30 & 90.25$\rightarrow$90.40 & 97.90$\rightarrow$98.02  & \multicolumn{4}{c}{92.25$\rightarrow$89.90}                                                                 \\ \hline
% Private Accuracy         & 1.46$\rightarrow$0.87  & 49.92$\rightarrow$42.86 & 3.08$\rightarrow$0.84    & 70.30$\rightarrow$61.33 & 69.46$\rightarrow$60.43 & 69.41$\rightarrow$59.03 & 98.75$\rightarrow$55.86
% \end{tabular}
% }
% \end{table}











==> ToDo.tex <==


\mohammad{the above does not hold for half-gaussian because sum of half-gaussian random variables is not half Gaussian, so we do not have a case for reLU.}



% \begin{itemize}

%     \item define a metric for correlation of public and private attributes
%     \begin{itemize}
%         \item provide an upper bound for what can be done
%         \item in experiments, use label overlap as a measure of correlation
%         \item rate distortion theory
%     \end{itemize}
    
%     \item Experiments:
%     \begin{itemize}
%         \item Diff privacy (noise adding method in case we didn't find diff privacy papers)
%         \begin{itemize}
%             \item Result: with same energy of noise added, we get better tradeoff between accuracy and privacy because we're adding a smarter noise to remove useless content rather than just adding random noise. 
%             \item two types: 1) add noise during training, 2) add noise after training. case 1 needs modified training whereas we don't need. Case 2 doesn't work or is very weak. 
%             \item plot: privacy vs accuracy for case 1, case 2, ours 2 (with different noise)
%         \end{itemize}
%     \end{itemize}
% \end{itemize}

==> others.tex <==
abstract:

% private cloud-based inference on data generated on edge devices is important. 
% \item Current methods for providing the privacy assume that the private attribute is known and the model is trained to minimize the leakage of secret information. 
% \item Current methods for providing the privacy assume a black-list of attributes to be censored from model representations, to minimize unintended information leakage.
% \item Current methods for providing the privacy train the model to obfuscate the private information and so assume the knowledge of a set of private attributes. 
% \item Current methods for providing the privacy train the model to filter out a black-list of private attributes and so assume that the knowledge of a set of private attributes. 
% \item assume that the private attribute is known and the model is trained to minimize the leakage of secret information. 
% train the model to filter out a black-list of private attributes and so assume that the knowledge of a set of private attributes. 

original abstract:
We introduce the notion of null-space content in neural network representations.
% : information that is disregarded by the layers following the feature vector. 
% We empirically show that neural networks contain massive null-space content in their representations. 
The null-space content of features is disregarded by the neural network when performing the intended task but can be utilized to extract unintended information. For instance, features extracted by a gender classifier (intended attribute) can be used to identify race (unintended label). We show that filtering out the null-space information helps provide privacy in cloud-based neural network inference while preserving utility, e.g., obfuscate race while preserving gender classification accuracy. We formulate the null-space content only based on the intended attribute, without incorporating private label(s). \edit{Although this assumption is much stricter than contemporary research, we empirically show that filtering null-space content outperforms prior work in terms of utility and privacy.}



For instance, a smart speaker that has been trained to obfuscate the speaker's gender and age will fail to censor the speaker's mood or the background talk or music. 
The need for identifying all possible private attributes and assembling the required training data is a limiting factor for deploying private cloud inference. 

It then decomposes its output into signal- and null-space components of the server network, and removes the null-space content before sending it to the server. 
The edge device can further remove the low-energy components of the signal-space to improve the privacy at the cost of reducing the accuracy on the main task.
